Eulerian graphs and local complementation

We define pure graphs, invertible graphs, and the notion of complementation of bicoloured graphs. The study of pure graphs is motivated by two conjectures about the transition systems of eulerian graphs and by the Cycle Double Cover Conjecture. We show how substitution rules can be used to determine when two complementation words produce the same graph. For bicoloured graphs, complementation words give way to complementation sets. The invertible graphs (bicoloured graphs whose vertex set is a complementation set) are shown to have the property that their inverse has the same automorphisms. The property of being invertible can also be defined for non-coloured graphs by endowing them with their natural colouring. It is proposed that a characterization of pure graphs would contribute to establish the truth of the Cycle Double Cover Conjecture. We show how pure graphs have essential factorizations into primitive pure graphs. The four primitive pure parity classes are presented.

==> temp.tex <==
Avant tout, je tiens à remercier mon directeur de recherche, Gert Sabidussi. Au cours de nos entretiens, j'ai apprécié sa rigueur de raisonnement et son caractère franc et jovial. Ces années de recherches ont comporté leur part de doutes et si j'ai mené ce travail à terme, c'est en grande partie parce qu'il m'a traité en collègue.

Je remercie Marie-France, ma compagne, que j'admire.

Comme d'autres avant moi, je remercie Jérome Fournier, qui sait mettre les gens à l'aise et contribue beaucoup à rendre l'atmosphère du département accueillante. 

